Cardinality constrained submodular maximization for random streams

We consider the problem of maximizing submodular functions in single-pass streaming and secretaries-with-shortlists models, both with random arrival order. For cardinality constrained monotone functions, Agrawal, Shadravan, and Stein gave a single-pass $(1-1/e-\varepsilon)$-approximation algorithm using only linear memory, but their exponential dependence on $\varepsilon$ makes it impractical even for $\varepsilon=0.1$. We simplify both the algorithm and the analysis, obtaining an exponential improvement in the $\varepsilon$-dependence (in particular, $O(k/\varepsilon)$ memory). Extending these techniques, we also give a simple $(1/e-\varepsilon)$-approximation for non-monotone functions in $O(k/\varepsilon)$ memory. For the monotone case, we also give a corresponding unconditional hardness barrier of $1-1/e+\varepsilon$ for single-pass algorithms in randomly ordered streams, even assuming unlimited computation. Finally, we show that the algorithms are simple to implement and work well on real world datasets.

==> paper/checklist.tex <==
\section*{NeurIPS Checklist}

\begin{itemize}
    \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? {\bf Yes.}
    \item Have you read the ethics review guidelines and ensured that your paper conforms to them? {\bf Yes.}
    \item Did you discuss any potential negative societal impacts of your work? {\bf Not applicable to this work, as it is mostly a theoretical analysis of the approximation ratio for a particular algorithm.}
    \item Did you describe the limitations of your work? {\bf Partially. The experiments compares (and loses) against a strong offline algorithm (Section 5). The limitations of the random order streaming model is discussed in prior works and is a commonly used model, so we did not address modeling limitations directly.}
    \item Did you state the full set of assumptions of all theoretical results? {\bf Yes. See Section 1.1.}
    \item Did you include complete proofs of all theoretical results? {\bf Yes. See supplemental.}
    \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? {\bf Yes. See supplemental, Section D.}
    \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? {\bf Yes. See experimental sections in supplemental and main paper.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? {\bf Yes. See shaded regions for Figure 1.}
    \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? {\bf Yes. See Section 5.}
\end{itemize}
All other questions (e.g. ones regarding human subjects) were not applicable to this work.



==> paper/old-lower-bound.tex <==


\section{$1-1/e+\eps$ hardness instances for monotone submodular maximization}
\begin{theorem}
Any algorithm that remembers fewer than $\varepsilon n$ elements
does not obtain a $\left(1-1/e+O(\varepsilon)\right)$-approximation
with high probability.
\end{theorem}

\begin{proof}
For parameters $r<k<n$, Nemhauser and Wolsey~\cite{NW78Bound} construct
a submodular function $f=f_{r,k,n}$ over a ground set of $\Theta(n)$
elements, of which a subset $S$ of $k$ elements is called {\em special},
such that the following properties hold:
\begin{enumerate}
\item $f(S)=1$.
\item $f(T)\leq1-1/e+O\left(r/k\right)$ for any set $T$ of $\le k$ elements
such that $\left|S\cap T\right|\le r$.
\item For any set $T'$ with $\le r$ special elements, $f\left(T'\right)$
depends only on $\left|T'\right|$.
\end{enumerate}
In particular, the last property implies that as long as our algorithm
never stores more than $r$ special elements, it cannot distinguish
between special and non-special elements. 

We use the above construction with $r:=2\varepsilon k$. If the algorithm
remembers a random subset of $\le\varepsilon n$ elements, in expectation
only $\varepsilon k$ of them will be special; with exponentially
high probability, the number of stored special elements is at most
twice that, aka $\le r$. Therefore, if by time step $T$ the algorithm
hasn't queried a set with more than $r$ special elements, the elements
will continue to be indistinguishable to the algorithm, and thus the
elements stored in time step $T+1$ will continue to be an almost\footnote{This subset is not completely uniform because we sample elements without
replacement, and we condition on not having seen a subset with $>r$
special elements in previous time steps. Because the latter event
happens with probability almost one, this has negligible effect on
distribution.} uniformly random subset of $\le\varepsilon n$ elements. Since the
probability of storing $>r$ special elements in any time step is
exponentially small, we can take a union bound over all $n$ time
steps. Therefore, with high probability the algorithm will return
a set $T$ satisfying 
\[
f(T)\leq1-1/e+O\left(\underbrace{r/k}_{=2\varepsilon}\right). \qedhere
\]
\end{proof}

\begin{theorem}
In the oracle query model, for all $\epsilon>0$, any algorithm (with unbounded computational power) that achieves $1-\frac{1}{e}+\epsilon$ approximation on the max-coverage problem requires memory enough to store $\Omega(\frac{n}{k^{3/2}})$ sets.
\end{theorem}
\begin{proof}
We first construct the set system for our hard instance.
The universe of elements is a $n$-dimensional hypercude $[k]^n$.
Let $R_{i}$ denote the set $\{\mathbf{x}\in[k]^n \mid x_i=1\}$, namely, the set of all the vectors of which the $i$-th coordinate is $1$. Let $S_{i}$ denote the set $\{\mathbf{x}\in[k]^n \mid x_1=i,\,x_2\neq k\}\cup \{\mathbf{x}\in[k]^n \mid x_1=k,\,x_2=k\}$.
Our set system consists of $k$ good sets $S_1,\dots,S_k$ and $n-k$ bad sets $R_{k+1},\dots,R_{n}$. We make the following three observations:
\begin{itemize}
    \item For any $r\in[n-k]$ and $s\in\{0,1,2\}$, any distinct $i_1,\dots,i_r\in \{k+1,\dots,n\}$ and $j_1,j_2\in[k]$, we have that $$|(\cup_{t=1}^{r} R_{i_t})\cup (\cup_{t=1}^{s} S_{j_t})|=\left(1-\left(1-\frac{1}{k}\right)^{r+s}\right)k^n.$$
    \item Moreover, it holds that $$|\cup_{t=1}^{k} S_{j_t}|=\left(1-\frac{1}{k}+\frac{1}{k^2}\right)k^n.$$
    \item Finally, the output of the coverage function is fully determined by the number of good sets and the number of bad sets in the input. Hence, there is a succinct encoding of all the possible values of this coverage function, which uses $O(\log n)$ bits.
\end{itemize}

Next, we show that any algorithm that stores $o(\frac{n}{k^{3/2}})$ sets can have at most one good set in its memory with high probability whenever a good set shows up in the stream. This is proved by induction on the number of good sets that have appeared in the stream. For the base case, this is obviously true when the first or the second good set appears. For the induction step, for $j\ge 2$, let $E_j$ denote the event that for all $t\le j$,
the algorithm remembers at most one good set when the $t$-th good set shows up in the stream, and let $p_j$ be the probability that $E_j$ happens (note that $p_2=1$). Conditioned on $E_j$, when the $j$-th good set $S_{\sigma(j)}$ appears, there is at most one good set $S_{\sigma(i)}$ in the memory, where $\sigma$ is a random permutation because of the random order model. Since there are only two good sets $S_{\sigma(i)},S_{\sigma(j)}$ among the sets stored by the algorithm when the $j$-th good set appears and all the sets appearing since the $j$-th good set and before the $(j+1)$-th good set in the stream, by the first observation above, the coverage function is completely symmetric with respect to all these sets, and hence, the two good sets are indistinguishable from the bad sets.
Therefore, from the perspective of the algorithm, each of these sets has probability $\frac{k}{n}$ being a good set, and hence, when the $(j+1)$-th good set shows up, the algorithm stores $o(\frac{n}{k^{3/2}})$ sets, and the probability that an arbitrary pair of sets in the memory is good is roughly $\frac{k^2}{n^2}$. By union bound over all pairs, the probability that there exists a pair of good sets in the memory conditioned on $E_j$ is $o(\frac{1}{k})$. Therefore, when the $(j+1)$-th good set appears in the stream, the probability that there are $\le 1$ good set in the memory conditioned on $E_j$ is at least $1-o(\frac{1}{k})$, namely, $p_{j+1}\ge p_j(1-o(\frac{1}{k}))$. It follows by continuing the induction steps that the probability that $E_n$ happens is $1-o(1)$. Hence, the algorithm has at most $2$ good sets with high probability at the end of stream.

Now we upper bound the approximation ratio attained by the union of $k-2$ bad sets and $2$ good sets chosen by the algorithm. By the second observation in the first paragraph, the optimum of our instance is at least $(1-\frac{1}{k}+\frac{1}{k^2})k^n$ achieved by the $k$ good sets. By the first observation in the first paragraph, any $k-2$ bad sets and $2$ good sets together have value
\[
    \left(1-\left(1-\frac{1}{k}\right)^{k}\right)k^n,
\]
and thus, the approximation ratio is at most
\begin{equation}
\frac{1-(1-\frac{1}{k})^{k}}{1-\frac{1}{k}+\frac{1}{k^2}},
\end{equation}
which approaches $1-\frac{1}{e}$ asymptotically, as $k$ increases.
\end{proof}

==> todolist.tex <==
\section*{Todo list}
\begin{itemize}
\item
We can improve the analysis to show that the approximation factor is $\frac1 k\frac{1-(1-1/k)^{2k}}{1-(1-1/k)^2}$, which actually gets a clean $1/2(1-1/e^2)$ I think. Analysis to be done.
\item
Does our result also apply to the submodular secretary model? Seems like we're using a ``shortlist" of size $\beta k$ (this is the history). We can also apply the approximate maximum finding algorithm of ~\cite{SMC19} to reduce the shortlist overhead of finding the argmax.
\item
Replace $w_i$ with $W_i$ and etc ($w_j$, $w_{i_j}$, $w_k$) and $W_i$ with $\mathcal{W}_i$ for more pleasant notation.
\item
Sub-sampled continuous greedy version?
\item
Add remark showing the previous submodular shortlists paper has bad dependence on k
\item
This also applies to set cover in $\tilde{O}(k)$ memory in a {\it single} pass, if we use $F_0$ estimation techniques to store the sets. I think this is a new result. (Note in the streaming model, its not trivial to store the ``elements" of the optimal solution, since that could take up to $O(n)$ memory). 
\item
$1/e$ for non-monotone cardinality constrained? Seems like we could try to apply the algorithm of Buchbinder '14 directly (Take top $k$ residuals, plus dummy elements if some residuals are $< 0$. Choose one at random to add to the solution) 
\item
Change to $\mathcal{H}_i$-compatible instead of $i$-compatible.
\item
Remove $O(1/k)$ term from local search.
\item
We should also be able to do a simple algorithm for the non-monotone matroid case.
\end{itemize}

